RECKON: Large-scale Reference-based Efficient Knowledge Evaluation for Large Language Model

As large language models (LLMs) advance, efficient knowledge evaluation becomes crucial to verifying their capabilities. Traditional methods, relying on benchmarks, face limitations such as high resource costs and information loss. We propose the Large-scale Reference-based Efficient Knowledge Evaluation for Large Language Model (RECKON), which directly uses reference data to evaluate models. RECKON organizes unstructured data into manageable units and generates targeted questions for each cluster, improving evaluation accuracy and efficiency. Experimental results show that RECKON reduces resource consumption by 56.5% compared to traditional methods while achieving over 97% accuracy across various domains, including world knowledge, code, legal, and biomedical datasets. Code is available at https://github.com/MikeGu721/reckon

==> latex/00.Introduction.00.tex <==
Assessing the quality of text generated by language models has been a challenging task for a long time~\cite{chang2024survey}. 
Traditional approaches rely on a large amount of manually annotated ground truth benchmarks~\cite{hendrycks2020measuring, huang2024c, gu2024xiezhi} as well as n-gram automatic evaluation metrics~\cite{papineni2002bleu, lin2004rouge, banerjee2005meteor} used to align the ground truth and generated text. 
However, these metrics, primarily word co-occurrence-based, have been shown to neglect semantics and are insufficient in identifying factual inaccuracies.
The demanding cost of annotation and the limitations of n-gram automatic evaluation metrics make it difficult to evaluate open-ended results in various knowledge-intensive domains.


\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.99\linewidth]{latex//figs/arr_intro.png}
    \includegraphics[width=0.99\linewidth]{latex/figs/zhanglin_intro.pdf}
    \caption{The effect of external reference.}
    \label{fig:intro}
\end{figure}

With impressive text comprehension and instruction-following capabilities, ``Large Language Model~(LLM) as Evaluator'' has emerged as a solution to address the previously mentioned evaluation challenges to some extent~\cite{bai2024benchmarking, zheng2024judging, chan2023chateval}.
Existing research~\cite{bai2024benchmarking, li2024treeeval} enables LLMs to generate domain-specific questions by starting from predefined terms or keywords and iteratively refining the questions based on model responses.
However, these approaches overlook a crucial issue: 
\textbf{the knowledge within Evaluator LLM is limited, incomplete, and often outdated.}

To address the limitations and outdated knowledge in LLMs, it is natural to consider using external reference~\cite{van2024field, xie2023adaptive}. As shown in Fig. \ref{fig:intro}, the reference text corrected the model's original misjudgments.
However, this approach introduces several challenges for Evaluator LLMs:
(1) The length of the external references often far exceeds the processing capacity of the LLM, rendering it extremely challenging for the model to handle and utilize such vast amounts of information effectively.
(2) Evaluating external references consisting of exceptionally long texts demands a substantial amount of computational resources, which complicates efficiency and scalability in practical applications.
(3) Considering that LLMs are sensitive to the prompts, it is challenging to present accurate evaluation results based on references with diverse expressions.

To better integrate large volumes of external reference data into the assessment process effectively, we propose the \textbf{Reference-based LLM-as-Evaluator framework (Ref-Eval)} in this paper. 
Ref-Eval synthesizes external reference materials into discrete, manageable knowledge units. These units are organized into clusters, each associated with representative questions formulated to probe the evaluated model.
To enhance the comprehensiveness and precision of the evaluation, Ref-Eval identifies knowledge units that elicit ambiguous or omitted responses. These units are emphasized in subsequent interactions through carefully tailored questions.



We conduct experiments on multiple domain-specific text datasets. 
The experimental results indicate that Ref-eval achieves a consistency of more than 96\% with human results.
Compared to the theoretical best method, our method saves 55.9\% in money expense and saves 10k dollars in our dataset of 18M tokens. 
Ref-eval also provides instructive performance characteristics of models on real-world knowledge, for example, knowledge with brief or complex content and models with different capacities of in-context learning~\cite{min2022rethinking}. 


==> latex/00.Introduction.01.tex <==
Assessing the quality of text generated by language models has been a challenging task for a long time~\cite{chang2024survey}. 
Traditional approaches rely on a large amount of manually annotated ground truth benchmarks~\cite{hendrycks2020measuring, huang2024c, gu2024xiezhi} as well as n-gram automatic evaluation metrics~\cite{papineni2002bleu, lin2004rouge, banerjee2005meteor} used to align the ground truth and generated text. 
However, these metrics, primarily word co-occurrence-based, have been shown to neglect semantics and are insufficient in identifying factual inaccuracies.
The demanding cost of annotation and the limitations of n-gram automatic evaluation metrics make it difficult to evaluate open-ended results in various knowledge-intensive domains.


\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.99\linewidth]{latex//figs/arr_intro.png}
    \includegraphics[width=0.99\linewidth]{latex/figs/zhanglin_intro.pdf}
    \caption{The effect of external reference.}
    \label{fig:intro}
\end{figure}

With impressive text comprehension and instruction-following capabilities, ``Large Language Model~(LLM) as Evaluator'' has emerged as a solution to address the previously mentioned evaluation challenges to some extent~\cite{bai2024benchmarking, zheng2024judging, chan2023chateval}.
Existing research~\cite{bai2024benchmarking, li2024treeeval} enables LLMs to generate domain-specific questions by starting from predefined terms or keywords and iteratively refining the questions based on model responses.
However, these approaches overlook a crucial issue: 
\textbf{the knowledge within Evaluator LLM is limited, incomplete, and often outdated.}

To address the limitations of knowledge within LLMs, it is intuitive to consider incorporating external references~\cite{van2024field, xie2023adaptive}. As shown in Fig. \ref{fig:intro}, the reference text can correct the model's original misjudgments, providing a more accurate basis for evaluation. 
However, integrating external references into the LLM's evaluation process introduces several challenges. 
(1) The length of external references often exceeds the LLM's processing capacity, making it difficult for the model to extract relevant information efficiently. 
(2) Analyzing extensive reference materials demands significant computational resources, which raises concerns about scalability and efficiency in practical applications. 
(3) Due to the LLM's sensitivity to prompts, ensuring consistent and accurate evaluations across references with varying expression styles is challenging. 
These challenges must be addressed to unlock the full potential of using external references in LLM evaluations.


To overcome these challenges, we propose the \textbf{Ref}erence-based LLM-as-\textbf{Eval}uator framework (\textbf{Ref-Eval}).
Ref-Eval is designed to effectively manage and utilize large volumes of external reference by decomposing them into discrete, manageable knowledge units. 
These units are organized into clusters based on their thematic content, and the evaluation process involves generating targeted questions for each cluster to assess the performance of the model being evaluated.
The evaluation focuses on whether the responses adequately cover all relevant knowledge units within each cluster, thereby ensuring the comprehensiveness and precision of the assessment.
Any knowledge units that remain unaddressed, indicating that the evaluated model’s accuracy cannot be determined, are regrouped for further questioning in subsequent rounds. 
By adopting this iterative clustering and questioning approach, Ref-Eval not only mitigates the limitations of the LLM’s internal knowledge but also enhances the robustness of the evaluation process by efficiently leveraging the rich information contained in external references, thereby reducing the overall evaluation overhead.

% To overcome these obstacles, we propose the \textbf{Reference-based LLM-as-Evaluator framework (Ref-Eval)}. 
% Ref-Eval is designed to effectively manage and utilize large volumes of external reference data by breaking them down into discrete, manageable knowledge units. 
% These units are organized into clusters by their topics, with each cluster associated with specific questions designed to probe the model's performance. By systematically focusing on ambiguous or omitted responses, Ref-Eval ensures that the evaluation is both comprehensive and precise. This framework not only mitigates the limitations of LLM's internal knowledge but also enhances the robustness of the evaluation process by leveraging the rich information contained in external references.



We conduct experiments on multiple domain-specific text datasets. 
The experimental results indicate that Ref-eval achieves a consistency of more than 96\% with human results.
Compared to the theoretical best method, our method saves 55.9\% in money expense and saves 10k dollars in our dataset of 18M tokens. 
Ref-eval also provides instructive performance characteristics of models on real-world knowledge, for example, knowledge with brief or complex content and models with different capacities of in-context learning~\cite{min2022rethinking}. 


==> latex/00.Introduction.02.tex <==
\gzh{主要修改思路：
1. 换故事，Boundaries根本不重要，Ref-Eval应该要重视以下几点：

文章主要的卖点：
- 评估应当从信息源直接出发——减少构建benchmark所带来的开销，以及随之而来的评估领域的局限和评估方法上的局限。

从信息源出发的评估的难点：
- 数据量大且内容杂乱，所以需要有效整理，从而才能进行准确的评估——在CommonsenseReasoning上进行实验，用更少的token取得和Benchmark-Based Evaluation差不多的结果
- 信息源和LLM记忆可能相悖，需要能以reference为准——在UncommonsenseReasoning上进行实验
- 适合不同的reference类型——就现有的实验足够了

2. 补实验结果，如上

3. 方法部分改写
- 虽然被审稿人argue了，但我感觉写得还挺容易看懂；让本科生同学看一遍吧，如果他能看懂，就象征性改改就行了。

4. 全文writing的改写

}


Assessing the quality of text generated by language models has been a challenging task for a long time~\cite{chang2024survey}. 
Traditional approaches rely on a large amount of manually annotated ground truth benchmarks~\cite{hendrycks2020measuring, huang2024c, gu2024xiezhi} as well as n-gram automatic evaluation metrics~\cite{papineni2002bleu, lin2004rouge, banerjee2005meteor} used to align the ground truth and generated text. 
However, these metrics, primarily word co-occurrence-based, have been shown to neglect semantics and are insufficient in identifying factual inaccuracies.
The demanding cost of annotation and the limitations of n-gram automatic evaluation metrics make it difficult to evaluate open-ended results in various knowledge-intensive domains.


\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.99\linewidth]{latex//figs/arr_intro.png}
    \includegraphics[width=0.99\linewidth]{latex/figs/zhanglin_intro.pdf}
    \caption{The effect of external reference.}
    \label{fig:intro}
\end{figure}

With impressive language comprehension and instruction-following capabilities, ``Large Language Model~(LLM) as Evaluator'' has emerged as a solution to address the previously mentioned evaluation challenges to some extent~\cite{bai2024benchmarking, zheng2024judging, chan2023chateval}.
Existing researches~\cite{bai2024benchmarking, li2024treeeval} enables LLMs to generate domain-specific questions by starting from predefined terms or keywords and iteratively refining the questions based on model responses.
However, these approaches overlook a crucial issue: 
\blue{
\textbf{the knowledge within Evaluator LLM is limited, incomplete, and often outdated.}
}
\gzh{
换个表达，切一个具体的点，可以先把后面写好再来改这句话
}


To address the limitations of knowledge within LLMs, it is intuitive to consider incorporating external references~\cite{van2024field, xie2023adaptive}.
As shown in Fig. \ref{fig:intro}, the reference text can correct the model's original misjudgments, providing a more accurate basis for evaluation. 
However, integrating external references into the LLM's evaluation process introduces several challenges. 
\blue{(1) The length of external references often exceeds the LLM's processing capacity, making it difficult for the model to extract relevant information efficiently. }
\gzh{换个表达，现在主要讲的是reference的“长度”，换成使用reference的“开销”非常庞大，开销可以包括“单词数”、“计算力”、“API调用费用”等等}
\blue{(2) Analyzing extensive reference materials demands significant computational resources, which raises concerns about scalability and efficiency in practical applications.}
\gzh{第二点和第一点融合了，第二点可以换一个新的点：
如果reference和parameter memory冲突了，如何保证LLM能够按照reference来进行评估}
(3) Due to the LLM's sensitivity to prompts, ensuring consistent and accurate evaluations across references with \blue{varying expression styles is challenging. }
\gzh{
style不重要，重要的是如何在不同LLM的问答过程中，以及如何在不同domain的reference中依然保持consistent and accurate
}
\blue{
These challenges must be addressed to unlock the full potential of using external references in LLM evaluations.
}\gzh{这句话不要，多余的}


To overcome these challenges, we propose the \textbf{Ref}erence-based LLM-as-\textbf{Eval}uator framework (\textbf{Ref-Eval}).
Ref-Eval is designed to effectively manage and utilize large volumes of external reference by decomposing them into discrete, manageable knowledge units. 
These units are organized into clusters based on their thematic content, and the evaluation process involves generating targeted questions for each cluster to assess the performance of the model being evaluated.
The evaluation focuses on whether the responses adequately cover all relevant knowledge units within each cluster, thereby ensuring the comprehensiveness and precision of the assessment.
Any knowledge units that remain unaddressed, indicating that the evaluated model’s accuracy cannot be determined, are regrouped for further questioning in subsequent rounds. 
By adopting this iterative clustering and questioning approach, Ref-Eval not only mitigates the limitations of the LLM’s internal knowledge but also enhances the robustness of the evaluation process by efficiently leveraging the rich information contained in external references, thereby reducing the overall evaluation overhead.


We conduct experiments on multiple domain-specific text datasets. 
The experimental results indicate that Ref-eval achieves a consistency of more than 96\% with human results.
Compared to the theoretical best method, our method saves 55.9\% in money expense and saves 10k dollars in our dataset of 18M tokens. 
Ref-eval also provides instructive performance characteristics of models on real-world knowledge, for example, knowledge with brief or complex content and models with different capacities of in-context learning~\cite{min2022rethinking}. 


==> latex/00.Introduction.03.tex <==
As large language models (LLMs) continue to advance, knowledge evaluation has become a critical aspect of verifying their capabilities and driving improvements. Accurate knowledge evaluation ensures that LLMs can reliably perform tasks across diverse.
In high-stakes fields such as healthcare, education, and law, robust evaluation methods are essential to mitigate the risks of errors or outdated information. 
Evaluation serves to assess and ensure the alignment between model performance and established reference standards, facilitating quantitative measurement of model capabilities against verified ground truth data.
With the rapid expansion of LLM applications, the demands on knowledge evaluation have evolved. 
Evaluations now require broader coverage, more complex tasks, and the handling of significantly larger datasets, posing unprecedented challenges for traditional methods. 

% The essence of evaluation is to align the model's performance with golden reference data.
%reference data

%% 第一段——评估的本质：align模型的performance和reference data
%% 第二段——benchmark：对reference的改造/凝练
%%第三段——直接从reference出发的好处。challenge写成陈述句

Traditional knowledge evaluation typically relies on benchmarks, including formats such as multiple-choice questions, fill-in-the-blanks, and marking tasks. 
Benchmarks are essentially condensed or refined representations of reference data, designed to make evaluation manageable and systematic. 
While widely adopted, these benchmarks have inherent limitations. 
First, creating benchmarks is resource-intensive, requiring substantial human and computational effort. 
Second, simplifying complex, diverse information into standardized questions often leads to information loss, introducing biases or distorting the validity of evaluated knowledge. 
Finally, single benchmarks struggle to encompass the complexity and diversity of knowledge domains, limiting their adaptability and applicability. 
As evaluation requirements grow more extensive and intricate, traditional benchmark-based approaches increasingly fall short.
 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{latex/figs/arr_intro_1126.pdf}
    \caption{The comparison of different evaluation method.}
    \label{fig:intro}
\end{figure}

As illustrated in Fig. \ref{fig:intro}, relying on benchmarks makes evaluation resource-intensive, introduces biases by simplifying complex information, and struggles to adapt to the vast diversity of knowledge domains. In contrast, directly leveraging rich and dynamic reference data offers several advantages: it avoids the information loss inherent in predefined questions, reduces the high costs associated with benchmark creation, and provides greater flexibility to address diverse evaluation needs. However, this approach also introduces new challenges:
1）Reference datasets are often large and unstructured, making it difficult to organize and utilize them effectively in evaluations.
2）Without predefined questions or fixed answers, ensuring that a model’s output aligns consistently and fairly with the reference data becomes a significant challenge.

% 第四段——ref-eval是怎么解决challenge的，对应第三段

To address these challenges, we propose a novel framework called Reference-based evaluation (Ref-eval), which directly evaluates models using reference data. 
In response to the difficulty of organizing and utilizing large and unstructured reference datasets, Ref-eval decomposes the reference data into discrete, manageable knowledge units. 
 These units are then grouped into thematic clusters, forming an organized knowledge structure that streamlines the evaluation process. 
To solve the problem of ensuring consistent and fair alignment without predefined questions or fixed answers, Ref-eval generates targeted questions for each knowledge cluster.
The evaluation focuses on assessing whether the model’s responses adequately cover all relevant knowledge units, ensuring comprehensiveness and accuracy.


%第一句应该是观点/结论
Experimental results \blue{further}\gzh{No ``further''} demonstrate the superiority of Ref-eval, confirming it as a comprehensive, efficient, and adaptable framework for knowledge evaluation.
Across various common-sense and non-common-sense reasoning tasks, Ref-eval significantly reduced computational resource usage while achieving comparable or even superior evaluation accuracy to traditional benchmark-based methods. 
\blue{For instance,}\gzh{Don't use ``for instance''} \blue{in a specific reasoning task}\gzh{Detail it, in which specific task.}, Ref-eval reduced resource consumption by 56.5\% while maintain \blue{the same}\gzh{the same as ?} evaluation accuracy. 
Moreover, \blue{Ref-eval demonstrated excellent adaptability to reference of deffierent domains, making it simple and versatile to use.}\gzh{detail performance should be written here to demonstrate your claim} 

% 除此之外，ref-eval展现出xxx能力

==> latex/02.Method.00.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figs/method.pdf}
    \caption{\method~consists of five main components that form a cycle of assessment.}
    \label{fig:method}
\end{figure*}




As shown in Fig.\ref{fig:method}, \method~consists of five main components, and the description of these components is as follows:

\textbf{Step 1 Preparing Knowledge Unit Candidates:}
The \method~ framework begins by preparing knowledge units that will be utilized throughout the evaluation process. These units are sourced primarily from two places: external references or knowledge units that should have been covered in previous evaluation rounds.

\textbf{Step 2 Clustering:}
Once the initial knowledge units are collected, the next step is to cluster these units.
Clustering is performed to effectively organize knowledge units into coherent groups to facilitate the evaluation process. This organization is achieved by analyzing the semantic relationships between different knowledge units. Each knowledge unit, which may consist of facts, concepts, and information relevant to the related field, is transformed into an embedding representation. These units are then classified based on the proximity of their embeddings in semantic space, effectively creating subsets of knowledge that are thematically related.


\textbf{Step 3 Question Generation:}
\method~leverages an LLM to generate questions for each cluster.
This step utilizes the capabilities of the language model to pose questions that are not only relevant to the theme of the cluster but also aimed at probing the depth and accuracy of the presented knowledge.
The questions are slightly adjusted during the evaluation based on the responses provided by the language model being evaluated to uncover any inconsistencies or gaps in the model's understanding of the given references.
The questions are slightly adjusted during the evaluation due to the response made by the evaluated language model, which aims to uncover any inconsistencies or gaps in the language model's understanding of the given reference.



\textbf{Step 4 Get Response:}
In this phase, the evaluator gets the response from the other evaluated targets.
These responses are crucial as they represent the model's current understanding and knowledge.
The \method~ analyzes these responses to determine the model's proficiency and the accuracy of the information it provides. 
If responses are found missing the point of the question, \method~will continue to prompt the model to generate questions to cover the relevant knowledge units.

\textbf{Step 5 Judging:}
The final step involves instructing the evaluation LLM to assess the extent to which the evaluated model's responses cover the specified knowledge units. 
In this phase, \method~ labels the covered knowledge units as either correct or incorrect. 
For knowledge units that remain uncovered by the evaluated model's response, \method~identifies and retains them for reorganization and re-evaluation. 
The process starts again from the initial step in subsequent assessment rounds.

The details of each step, including the prompts, models, inputs, and outputs, are provided in \ref{A.1}.

% The final step involves a detailed evaluation of responses using a combination of automated and manual review methods to assess the correctness, relevance, and depth of the response provided by the language model. 
% This step is iterative, with each round of questioning and answer review refining the model's understanding of both known and unknown content.
% Through this continuous cycle, \method~identifies and retains unresolved knowledge units, prioritizing them in subsequent evaluations to progressively improve the accuracy and comprehension capabilities of the model.





==> latex/05.Analysis.00.tex <==
\input{latex/table_tex/corr_table.1}

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row height for better spacing
\fontsize{9}{6}\selectfont
\begin{tabular}{|p{0.45\textwidth}|}
\hline
\textbf{Question:} What was the Silent Holy Stones' director award in 2005? \\
\textbf{Answer:} Directed by Pema Tseden, won the Golden Rooster Award for Best Directorial Debut in 2005, marking a significant step for Tibetan cinema. \\
\textbf{Judgement:} \textcolor{red}{Incorrect} \\
\hline
\textbf{Reference Text:} The Silent Holy Stones was nominated in the \textbf{Best Director category in the 2005 Beijing College Student Film Festival}. \\
\hline
\end{tabular}
\caption{Performance of GPT-4 on Uncommon Dataset by \method.}
\label{tab:performance_ref_eval_uncommon}
\end{table}


\input{latex/table_tex/consumption_table.2}
\input{latex/table_tex/performance_table.2}


% \subsection{Evaluation Result of Different LLMs}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.87\linewidth]{latex/figs/question_classification.png}
    \vspace{-3mm}
    \caption{The counts of 6 types of questions of \method~used for different models.}
    \label{fig:question_classification}
\end{figure*}
% By detecting the model performance on different LLMs by \method, there are some important discoveries:

\begin{table}[]
\small
\centering
\begin{tabular}{@{}l|cccccc@{}}
\toprule
           & Code   & Legal.term & Wiki   & Med.rand  \\ \midrule
Jw/oR & 97.2  & 95.5     & 72.6 & 90.9    \\
\method~  & 95.4 & 90.9     & 54.5  & 82.1    \\ \bottomrule
\end{tabular}
\caption{Evaluation with and without reference.}
\label{tab:wo}
\end{table}

\begin{table}[]
\centering
\small
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{l}{\cellcolor{mygray} Model Accuracy}                       \\ \midrule
\multicolumn{1}{l|}{}           & GPT4 & GPT3.5 & LLaMA2 \\ \midrule
\multicolumn{1}{l|}{\method}   & 31.7 & 32.8   & 24.7   \\ \midrule
\multicolumn{1}{l|}{Jw/oR} & 84.4 & 87.3   &    67.5   \\ \midrule\midrule
\multicolumn{4}{l}{\cellcolor{mygray} Reference Adherence Rate}                  \\ \midrule
\multicolumn{1}{l|}{}           & GPT4 & GPT3.5 & LLaMA2 \\ \midrule
\multicolumn{1}{l|}{\method}   &90.57 & 92.45 & 96.22\\\bottomrule
\end{tabular}
\caption{Evaluation performance on UnCommon.}
\label{tab:uncomman}
\end{table}


% \subsubsection{LLM Capacity}
\subsection{Evaluation Results}

\textbf{Models with larger parameters show greater precision and adaptability across diverse datasets, reflecting their ability to handle complex knowledge.}
As shown in Tab.\ref{tab:main1}, GPT-4 achieves the highest accuracy across all datasets, including 95.4\% on Code, 94.6\% on Legal.term, and 97.9\% on Med.sim.
These results highlight its exceptional adaptability and capability in handling both general and specialized tasks, particularly in biomedical fields. 
In comparison, GPT-3.5 achieves slightly lower accuracy, with 90.8\% on Legal.term and 54.5\% on Wiki, demonstrating that larger-scale models like GPT-4 outperform smaller ones in knowledge-intensive tasks.

% The results depicted in Tab.\ref{tab:main1} indicate that GPT4-turbo not only outperforms the competing models in each dataset but also exemplifies exceptional prowess in domains that demand specialized expertise, particularly in the biomedical field. 
% Its top accuracy underscores its robust adaptability and the impact of large-scale model architectures in handling complex queries and knowledge-intensive tasks.
% In contrast, although GPT3.5-Turbo performs well, its accuracy on the Legal.term and Wiki datasets is significantly lower than that of GPT4-Turbo. 
% \gzh{Lack of specific number of the experiment result in this paragraph.}

\textbf{Fine-tuning a model in specific domains significantly enhances its performance within those areas.}
PMC\_LLaMA, specifically designed for the biomedical domain, achieves relatively higher accuracy on Med.rand and Med.sim, with scores of 78.5\% and 75.7\%, respectively. While it does not outperform GPT-4, it shows clear advantages over general-purpose models like LLaMA2, which achieve only 73.2\% and 72.5\% on the same datasets. These results indicate that fine-tuning for specific domains significantly enhances a model’s ability to process specialized tasks effectively.

% PMC\_LLaMA is a model designed specifically for the biomedical field, and its architecture and parameters \blue{may}\gzh{this is a word with weak confidence.} be optimized for processing medical text and terminology. 
% As can be seen from the table, PMC\_LLaMA achieved relatively \blue{high}\gzh{higher than?} accuracy on the Med.rand and Med.sim datasets. 
% This shows that the model has significant advantages in processing medical-related tasks and may benefit from its specific training and fine-tuning in the biomedical field.
% \gzh{Lack of specific number of the experiment result in this paragraph.}

\subsection{Evaluation Performance with Reference Data}

\textbf{GPT4 tends to provide a `correct' judgment of the user's answer without external reference.} As shown in Tab.\ref{tab:wo}, the scores assigned to GPT-3.5 by Jw/oR are consistently higher than those by \method. However, manual verification reveals that the evaluation accuracy of \method~is higher than that of Jw/oR. This suggests that Jw/oR tends to overestimate by incorrectly evaluating wrong answers as correct, leading to inflated results. Further research revealed that the model tends to provide a `correct' judgment when it lacks understanding of the truly correct knowledge, likely due to the sycophantic tendencies present in RLHF-trained models.




\textbf{\method~makes evaluation more objective by strictly following reference text.}  
As shown in Tab.\ref{tab:performance_ref_eval_uncommon}, when evaluated using \method, GPT-4's response to the Uncommon dataset was marked as incorrect due to conflicts with the reference, even though the answer aligned with real-world knowledge. 
Specifically, GPT-4 correctly stated that the film \textit{``won the Golden Rooster Award for Best Directorial Debut in 2005.''} 
However, the Uncommon reference contradicts this, causing \method~to label the answer as `Incorrect'.  
In contrast, when using the model's own judgment (Jw/oR), GPT-4 achieved a high accuracy on the Uncommon dataset, as it answered questions based on real-world knowledge. 
This demonstrates the difference between \method's strict adherence to a reference and the model's own understanding. 
Manual verification further confirms that \method~follows the reference in over 90\% of cases, even when the reference contradicts the model’s internal knowledge.
% \gzh{you are repeating the analysis you have done before. This is nothing about the claim you've made in this paragraph.}
%%这段话我是想表达：根据LLM自己的判断（Jw/oR），GPTmodel在Uncommon上的正确率很高，但是如果用Uncommon的reference就是相反的



\subsection{Evaluation Performance Knowledge Clustering and Concept Characteristics}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figs/cluster30.png}
        \caption{k=30}
        \label{fig:subfig1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figs/cluster40.png}
        \caption{k=40}
        \label{fig:subfig2}
    \end{subfigure}
    \caption{The embedding map of the remaining knowledge units to be evaluated on the Wiki dataset in the process of evaluating GPT3.5-turbo at round \textbf{k} (k is different of the two sub-figures), where the representation of knowledge units of the same color is clustered in the same class, and their class names are displayed.}
    \label{fig:cluster}
\end{figure*}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\columnwidth]{latex/figs/frq_time.png}
    \caption{The frequency of knowledge units in multiple iterations of \method. The X-axis is the frequency of knowledge units, and the vertical axis is the number of knowledge units of a certain frequency.}
    \label{fig:frq_time}
\end{figure}

% \gzh{You changed words, but still, what is ``clear meaning'', and what is ``well-defined boundaries''? quantify them, use some machine learning words to describe Fig.~\ref{fig:subfig1}and Fig.~\ref{fig:subfig2}.}
\paragraph{Well-defined clusters of knowledge lead to a more effective evaluation by \method.} 
A cluster with low variance within the cluster and large distance between the clusters indicates a well-defined cluster. 
In Figure \ref{fig:subfig1}, the knowledge is divided into 13 distinct clusters with clear boundaries. 
Between rounds 30 (Figure \ref{fig:subfig1}) and 40 (Figure \ref{fig:subfig2}), clusters like ``Various films, TV shows, operas, and related media productions'' and ``Various STEM topics'' are fully evaluated by \method. 
These well-defined clusters enable precise question formulation and accurate model responses.
In contrast, clusters with unclear boundaries, such as \textit{ ``Various historical, biographical, electoral, media, educational and legal topics''}, are more difficult to evaluate. 
The broad range of topics within these clusters makes it difficult to ask questions with the same level of clarity and specificity as those within more clearly defined clusters, which can affect the accuracy of the evaluation.


\paragraph{Clustering greatly improves the efficiency of \method.}
Fig.\ref{fig:frq_time} illustrates the frequency distribution of repeated knowledge units in questions over multiple iterations.
The figure shows that as the frequency increases, the occurrence of `ignored' knowledge units (i.e., situations where the model fails to provide relevant answers) significantly decreases. 
This indicates that the clustering design in \method~effectively avoids high-frequency `ignored' knowledge units, thus generating questions from the same knowledge unit at a lower cost. 
This design helps ensure the diversity and relevance of questions, ultimately enhancing evaluation effectiveness.

\paragraph{LLMs exhibit better performance on knowledge units with concise and less complex content.}
Fig.~\ref{fig:frq_time} demonstrates that high-frequency `ignored' knowledge units typically contain extensive information. 
For example, \textit{``List of medical drama television programs worldwide''} includes a large amount of specific data.
This complexity leads to their frequent omission, especially when they are part of clusters with fewer informational knowledge units.
This behavior can be attributed to the characteristics of LLMs, which are more efficient at generating comprehensive answers to simpler, less information-dense knowledge units. 
In contrast, knowledge units that involve complex, detailed content tend to be `ignored' more often, as the model struggles to provide a succinct, yet accurate, response that covers all relevant aspects.
% It is obvious in Fig. \ref{fig:frq_time} that high-frequency "ignored" knowledge units tend to contain extensive information as they often represent multiple entities or lists.
% This contributes to their high frequency of being ignored, particularly when they are contained in a cluster with fewer informational knowledge units.
% This can be caused by the characteristics of LLMs, as they are more adept at giving a comprehensive answer, and the less informational knowledge units can be answered comprehensively with less text.
% }\gzh{I feel this is an important claim, but I didn't get the full meaning of this section.}

\input{latex/table_tex/case_table.1}
\subsection{Evaluation Performance of Different Types of Questions}

Fig.\ref{fig:question_classification} displays six types of questions with different interrogatives, each yielding varied outcomes in LLM responses.

%% 这样写可以吗？
% \textbf{The complexity of specific knowledge leads to poor performance in answering “who” and “where” questions.
% }
\textbf{LLMs consistently underperform on questions related to people and locations.}
Fig.\ref{fig:question_classification} shows that all models consistently performed poorly when tasked with answering `who' questions.
This difficulty likely stems from the fact that `who' questions often involve specific individuals, historical contexts, or cultural knowledge, which can be challenging for models to learn accurately.
Similarly, performance was also notably lower for questions related to location, i.e., the `where' question.
Models may struggle with disambiguation between different individuals sharing the same name, and they may not effectively handle nuanced information about various people.
This challenge could be attributed to the diverse contexts and geographical details that `where' questions often entail.

%% reasoning-based questions？
\textbf{\method~enables LLMs to realize their inherent potential.} 
By structuring questions with more contextual detail, \method~stimulates the model’s existing reasoning abilities, leading to improved performance on reasoning-based tasks. 
While models like GPT-4-turbo and LLaMa2-chat show better performance with Jw/R on `who' and `where' questions, which typically involve factual recall, \method's performance becomes comparable or superior with models like GPT-3.5-turbo. This shift is due to \method's ability to incorporate richer contextual information from related knowledge sources, enhancing the formulation of detailed and accurate questions. 
For example, in Tab.\ref{tab:case}, \method~triggers GPT-3.5-turbo's understanding of `damage' by providing relevant contextual clues, which helps improve response precision, whereas Jw/R may struggle without such context. 
This highlights the importance of comprehensive evaluation methods and the design of question generation prompts to avoid answer leakage, as explained in \ref{A.1}.
            
\subsection{Case Study} 

\textbf{\method~is more accurate than Jw/oR.}
As shown in the top case of Tab.\ref{tab:corr}, \method~uses a reference as the ground truth, while Jw/oR evaluates answers based on the knowledge within the LLM. 
For example, when asked about the opening time of Marino Railway Station, the answer is actually `Incorrect' according to Wiki. 
However, Jw/oR wrongly marks it as `Correct' based on the LLM’s outdated or inaccurate knowledge. 
In contrast, \method~correctly judges the answer as `Incorrect' and provides a credible explanation from the reference, demonstrating superior accuracy.

% \blue{
% \textbf{\method~stimulates the performance of LLMs with better in-context learning (ICL)~\cite{min2022rethinking} abilities.}}\gzh{try use the statement i write in review in previous susbsection} 
% Tab.\ref{tab:corr} demonstrates that Jw/R shows better performance compared to \method~with models like GPT4-turbo and LLaMa2-chat. 
% However, \method's performance becomes comparable or even superior with models such as GPT3.5-turbo. 
% \blue{
% This shift is primarily due to \method's ability to incorporate richer contextual information derived from related knowledge sources, which helps formulate more detailed and accurate questions. }\gzh{this statement is nearly the same as the previous section. remove it or change another reason.}
% For example, in Tab.\ref{tab:case}, we analyze the term \textit{'damage'}. \method~enriches GPT-3.5-turbo's understanding of 'damage' by providing contextual clues related to 'injury', thereby improving response precision. 
% Jw/R, however, may struggle without such context, underscoring the need for comprehensive evaluation methods.
% It is important to note that we design the question generation prompt to avoid leaking answers, as explained in \ref{A.1}.

% \textbf{\method~\blue{improve}\gzh{i don't think a evaluation method should ``improve'' the performance, but to show the real performance of a model. You need to change a word to represent it.} the performance of LLMs with better in-context learning~\cite{min2022rethinking} ability but poor knowledge memorizing.}
% % \gzh{
% % If \method~improves LLM with better ICL ability, I have a concern about whether \method~leaks answer.}
% %% We design the prompt of question generation to avoid leaking answers.
% Tab.\ref{tab:corr} demonstrates that Top-baseline shows better performance compared to \method~with models like GPT4-turbo and LLaMa2-chat.
% However, \method's performance becomes comparable or even superior with models such as GPT3.5-turbo.
% This shift is primarily due to \method's capability to incorporate richer contextual information derived from related knowledge sources, which facilitates more detailed and accurate question formulation. 
% For instance, in Tab.\ref{tab:case}, we analyze the term \textit{'damage'}. \method~enriches GPT-3.5-turbo's grasp of 'damage' with contextual clues on 'injury', improving response precision. Top-baseline can struggle without such context, highlighting the need for comprehensive evaluation methods.
% Notably, we design the prompt of question generation to avoid leaking answers in \ref{A.1}.


==> latex/table_tex/consumption_table.1.tex <==
\begin{table*}[ht]
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{@{}c|cc|cc|ccc@{}}
\toprule
& \multicolumn{2}{c|}{\textbf{Question Generation}} & \multicolumn{2}{c|}{\textbf{Response Judgment}} & \multicolumn{3}{c}{\textbf{All Consumption}}                     \\
&\#API-Call
&\#Token
&\#API-Call
& \#Token
& \#API-Call
& \#Token 
& \#Money~(US Cent) \\ \midrule
Ref-eval & 0.18               
& 44.9+105.21         & 1.1           & 315.7+422.3   & 1.3        & 360.6+527.5 & 1.9              \\
LLM(ref) & 1.0                & 215.5+240.8         & 1.0             & 318.0+368.5   & 2.0          & 533.6+609.3 & 2.7              \\ \bottomrule
\end{tabular}
}
\caption{The resource consumption of calling the API during the actual evaluation process of Ref-eval. The "\#API-Call" indicator indicates the average number of API calls required for each knowledge point; the "\#Token" indicator indicates the average number of tokens (input + output) required for each knowledge point; and the "\#Money" indicator indicates the average cost of calling the API for each knowledge point (in cent).}
\label{tab:effi}
\end{table*}

==> latex/table_tex/dataset_table.1.tex <==
\begin{table}[t]
\centering
\resizebox{0.99\columnwidth}{!}{\begin{tabular}{c|llccc}
\toprule
\textbf{Dataset}    & \textbf{Domain}           & \textbf{Source}     & \textbf{\#Words} & \textbf{\#Para.} & \textbf{\#Words in Para}. \\
\midrule
Comp       & Computer Science & CodeGPT\footnote{\url{https://github.com/zxx000728/CodeGPT/}}    & 2,371k  & 5,511          & 429.24  \\
Legal.term & Legal Terms      & Legalbench\footnote{\url{https://hazyresearch.stanford.edu/legalbench/}} & 233K   & 695           & 334.03  \\
Wikitext       & World Knowledge  & Wiki\footnote{\url{https://huggingface.co/datasets/wikitext}}       & 11,834k & 4,396          & 2,690.90 \\
Med.rand   & Biomedicine      & PubMedQA\footnote{\url{https://pubmedqa.github.io}}   & 877k   & 2,000          & 437.12  \\
Med.sim    & Biomedicine      & PubMedQA   & 351k   & 2,000          & 174.35 \\
\bottomrule
 \end{tabular}}
\caption{
Datasets information. \textbf{Comp} - Code-Text task of CodeGPT with computer science QA pairs. \textbf{Legal.term} - Definitions from Legalbench for law interpretation. \textbf{Wikitext} - High-quality Wikipedia articles. \textbf{Med.rand} and \textbf{Med.sim} - Subsets from PubMedQA, randomized and similarity-based (details in the Appendix).}
\label{tab:data}
\end{table}

==> latex/table_tex/performance_table.1.tex <==
\begin{table}[]
\centering
\resizebox{0.99\columnwidth}{!}{\begin{tabular}{l|lllll}
\hline
             & Comp            & Legal.term     & Wiki           & Med.rand       & Med.sim          \\\hline
GPT4-turbo   & \textbf{0.9545} &\textbf{0.9465} &\textbf{0.8267} &\textbf{0.9532} &  \textbf{0.9798}  \\
GPT3.5-turbo & 0.9292        &0.9088       &   0.5450       &    0.8211      &    0.8236           \\
LLaMA2-chat &   0.8312         &   0.8121       &    0.4290    &    0.7323            &   0.7258   \\
PMC\_LLaMA   &    --        &   --    &   --     &   0.7858            &  0.7572  \\ 
\hline
\end{tabular}}
\caption{The performance of the model on each dataset, expressed as accuracy, where the bold font indicates the highest accuracy.}
\label{tab:main1}
\end{table}
